A Reduced Order Approach for the Embedded Shifted Boundary FEM and a Heat Exchange System on Parametrized Geometries

A model order reduction technique is combined with an embedded boundary finite element method with a POD-Galerkin strategy. The proposed methodology is applied to parametrized heat transfer problems and we rely on a sufficiently refined shape-regular background mesh to account for parametrized geometries. In particular, the employed embedded boundary element method is the Shifted Boundary Method (SBM) recently proposed. This approach is based on the idea of shifting the location of true boundary conditions to a surrogate boundary, with the goal of avoiding cut cells near the boundary of the computational domain. This combination of methodologies has multiple advantages. In the first place, since the Shifted Boundary Method always relies on the same background mesh, there is no need to update the discretized parametric domain. Secondly, we avoid the treatment of cut cell elements, which usually need particular attention. Thirdly, since the whole background mesh is considered in the reduced basis construction, the SBM allows for a smooth transition of the reduced modes across the immersed domain boundary. The performances of the method are verified in two dimensional heat transfer numerical examples.

==> systeme.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "systeme"
\expandafter\edef\csname SYS@savedatcatcode\endcsname{\number\catcode`\@}
\catcode`\@11
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\SYSname                   {systeme}                             %
\def\SYSver                      {0.31}                              %
%                                                                    %
\def\SYSdate                  {2018/01/01}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% --------------------------------------------------------------------
% Author     : Christian Tellechea
% Status     : Maintained
% Email      : unbonpetit@netc.fr
% Package URL: https://www.ctan.org/pkg/systeme
% Bug tracker: https://framagit.org/unbonpetit/systeme/issues
% Repository : https://framagit.org/unbonpetit/systeme/tree/master
% Copyright  : Christian Tellechea 2017
% Licence    : Released under the LaTeX Project Public License v1.3c
%              or later, see http://www.latex-project.org/lppl.txt
% Files      : 1) systeme.tex
%              2) systeme.sty
%              3) systeme-fr.tex
%              4) systeme-fr.pdf
%              5) README
% --------------------------------------------------------------------
% --------------------------------------------------------------------

\def\SYS@newmacro#1{%
	\ifdefined#1%
		\errmessage{Package systeme Error: la macro \string#1\space existe deja. Contacter l'auteur svp.}%
	\fi
	\def#1%
}
\SYS@newmacro\SYSlongdate   {1\ier{} janvier 218}

\newtoks\SYS@systemecode
\newtoks\SYS@systempreamble

\newif\ifSYS@firstterm
\newif\ifSYS@sortvariable
\newif\ifSYS@star
\newif\ifSYS@extracol
\newif\ifSYS@autonum
\newif\ifSYS@followautonum
\newif\ifSYS@constterm

\newcount\SYSeqnum

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\ifdefined\xstringversion\else\def\SYS@nextaction{\input xstring.tex}\expandafter\SYS@nextaction\fi
	\immediate\write\m@ne{Package: \SYSname\space\SYSdate\space\space v\SYSver\space\space Saisie naturelle de systemes d'equations}%
	\newskip\normalbaselineskip \normalbaselineskip=12pt
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@firstofone#1{#1}
	\long\def\@gobble#1{}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\def\@empty{}
	\def\space{ }
\fi

% d\'efinit ce qu'est le s\'eparateur des \'equations par d\'efaut
\SYS@newmacro\syseqsep{\def\SYS@defaulteqsep}
\syseqsep{,}

% d\'efinit le coefficient pour l'espacement interligne
\SYS@newmacro\syslineskipcoeff{\def\SYS@lineskipcoeff}
\syslineskipcoeff{1.25}

% d\'efinit le signe qui marquera une colonne suppl\'ementaire \`a droite du tableau
\SYS@newmacro\sysextracolsign{\def\SYS@extracolsign}
\expandafter\sysextracolsign\expandafter{\string @}% on d\'efinit l'arobas avec le bon catcode.

% d\'efinit ce qui sera ins\'er\'e au d\'ebut et \`a la fin de la colonne suppl\'ementaire
\SYS@newmacro\syscodeextracol#1#2{\def\SYS@extracolstart{#1}\def\SYS@extracolend{#2}}
\syscodeextracol{\kern1.5em$}{$}

\SYS@newmacro\sysreseteqnum{\global\SYSeqnum\z@}

\SYS@newmacro\SYS@cslet#1{\expandafter\let\csname#1\endcsname}

% d\'efinit l'autonum\'erotation
\SYS@newmacro\sysautonum{\@ifstar{\SYS@followautonumtrue\SYS@autonum}{\SYS@followautonumfalse\SYS@autonum}}

\SYS@newmacro\SYS@autonum#1{%
	\ifx\@empty#1\@empty
		\SYS@extracolfalse
		\SYS@autonumfalse
	\else
		\SYS@extracoltrue
		\SYS@autonumtrue
		\def\SYS@autonumarg{#1}%
	\fi
}

% dimension qui sera ajout\'ee \`a la hauteur et \`a la profondeur du strutup ou strutdown
% ins\'er\'e \`a la premi\`ere et la derni\`ere \'equation
\SYS@newmacro\SYS@extrastrutdim{1.5pt}

% liste des signes devant \^etre compris comme signe d'\'egalit\'e s\'eparant les 2 membres de l'\'equation
\SYS@newmacro\SYS@equalsignlist{<=,>=,=,<,>,\leq,\geq,\leqslant,\geqslant}

\SYS@newmacro\sysaddeqsign#1{%
	\saveexpandmode\expandarg
	\IfSubStr{\expandafter,\SYS@equalsignlist,}{,#1,}
		\relax
		{\expandafter\def\expandafter\SYS@equalsignlist\expandafter{\SYS@equalsignlist,#1}}%
	\restoreexpandmode
}

% enl\`eve l'item #2 de la sc #1 qui contient une liste
\SYS@newmacro\SYS@removeiteminlist#1#2{%
	\saveexpandmode\expandarg
	\IfSubStr{\expandafter,#1,}{,#2,}
		{\StrSubstitute{\expandafter\@nil\expandafter,#1,\@nil}{,#2,},[#1]%
		\StrDel#1{\noexpand\@nil,}[#1]%
		\StrDel#1{,\@nil}[#1]%
		}%
		\relax
	\restoreexpandmode
}

\SYS@newmacro\sysremoveeqsign#1{%
	\SYS@removeiteminlist\SYS@equalsignlist{#1}%
	\SYS@removeiteminlist\SYS@equivsignlist{#1}%
}

% d\'efinit le signe d'\'egalit\'e #1 comme devant \^etre remplac\'e par #2 lors de l'affichage
\SYS@newmacro\sysequivsign#1#2{%
	\IfSubStr\SYS@equivsignlist{\noexpand#1,}\relax{\expandafter\def\expandafter\SYS@equivsignlist\expandafter{\SYS@equivsignlist#1,}}%
	\expandafter\def\csname SYS@equivsign@\string#1\endcsname{#2}%
}

\SYS@newmacro\SYS@equivsignlist{}

\sysequivsign{<=}\leq
\sysequivsign{>=}\geq

\SYS@newmacro\SYS@firstiteminlist#1,#2\@nil{#1}

\SYS@newmacro\SYS@removefirstiteminlist#1,{}

% #1 est l'\'equation courante. La macro la s\'epare en 2 membres -> \SYS@leftmember et \SYS@rightmember
% le signe de s\'eparation entre les 2 membres se trouve dans \SYS@currenteqsign
\SYS@newmacro\SYS@splitinmembers#1{%
	\def\SYS@leftmember{#1}\let\SYS@currenteqsign\@empty\let\SYS@rightmember\@empty
	\expandafter\SYS@splitinmembers@i\expandafter{\SYS@equalsignlist,}% parcourt \SYS@equalsignlist pour s\'eparer en 2 membres
	\IfSubStr{\expandafter,\SYS@equivsignlist}{\expandafter,\SYS@currenteqsign,}% si le signe est dans la liste des substitutions
		{\expandafter\let\expandafter\SYS@currenteqsign\csname SYS@equivsign@\detokenize\expandafter{\SYS@currenteqsign}\endcsname}% le remplacer
		\relax
}

% #1 est la liste des signes d'\'egalit\'e
\SYS@newmacro\SYS@splitinmembers@i#1{%
	\ifx\@empty#1\@empty
	\else
		\IfSubStr\SYS@leftmember{\SYS@firstiteminlist#1\@nil}% si l'\'equation contient un des signes
			{\expandafter\def\expandafter\SYS@currenteqsign\expandafter{\SYS@firstiteminlist#1\@nil}% sauvagarde le signe
			\StrBehind\SYS@leftmember\SYS@currenteqsign[\SYS@rightmember]% proc\`ede \`a la s\'eparation
			\StrBefore\SYS@leftmember\SYS@currenteqsign[\SYS@leftmember]% en deux membres
			\let\SYS@nextaction\relax
			}%
			{\def\SYS@nextaction{\expandafter\SYS@splitinmembers@i\expandafter{\SYS@removefirstiteminlist#1}}}% sinon, recommencer en enlevant le 1er signe
		\expandafter\SYS@nextaction
	\fi
}

\SYS@newmacro\SYS@ifcontains#1#2{%
	\def\SYS@ifcontains@i##1#2##2\@nil{\ifx\@empty##2\@empty\expandafter\@secondoftwo\else\expandafter\@firstoftwo\fi}%
	\SYS@ifcontains@i#1\@@nil#2\@nil
}

% analyse une \'equation et la d\'ecoupe en termes et signes
\SYS@newmacro\SYS@spliteqinterms#1{%
	\IfSubStr{\noexpand#1}\SYS@extracolsign% y a t-il un signe de colonne suppl\'ementaire ?
		{\StrBefore{\noexpand#1}\SYS@extracolsign[\SYS@leftmember]%
		\StrBehind{\noexpand#1}\SYS@extracolsign[\SYS@rightmember]%
		\SYS@cslet{SYS@extracol@\SYS@eqnumber}\SYS@rightmember
		\SYS@extracoltrue
		}%
		{\def\SYS@leftmember{#1}}%
	\expandafter\SYS@splitinmembers\expandafter{\SYS@leftmember}% trouver les membres de gauche et droite et le signe qui les s\'epare
	\unless\ifx\SYS@currenteqsign\@empty
		\SYS@cslet{SYS@eqsign@\SYS@eqnumber}\SYS@currenteqsign% stocker ce signe s'il existe
	\fi
	\IfBeginWith\SYS@leftmember\space{\StrGobbleLeft\SYS@leftmember\@ne[\SYS@leftmember]}\relax% pas d'espace pour commencer le membre de gauche
	\IfBeginWith\SYS@leftmember+% amputer le membre de gauche du premier signe et le stocker temporairement s'il existe et sinon...
		{\StrSplit\SYS@leftmember\@ne\SYS@currentsign\SYS@leftmember}%
		{\IfBeginWith\SYS@leftmember-%
			{\StrSplit\SYS@leftmember\@ne\SYS@currentsign\SYS@leftmember}%
			{\def\SYS@currentsign{+}}}% ce signe est "+"
	\SYS@spliteqinterms@i\@ne
	\SYS@cslet{SYS@right@\SYS@eqnumber}\SYS@rightmember
}

\SYS@newmacro\SYS@spliteqinterms@i#1{%
	\StrPosition\SYS@leftmember+[\SYS@posplus]%
	\StrPosition\SYS@leftmember-[\SYS@posminus]%
	\ifnum\numexpr\SYS@posplus+\SYS@posminus=\z@ % il n'y a ni "+" ni "-"
		\let\SYS@currentterm\SYS@leftmember% prendre tout ce qui reste
		\SYS@assignterm% et assigner ce dernier terme avec le dernier signe trouv\'e
	\else
		\edef\SYS@nextsign{\ifnum\SYS@posplus=\z@-\else\ifnum\SYS@posminus=\z@+\else\ifnum\SYS@posplus<\SYS@posminus+\else-\fi\fi\fi}% d\'ecider de ce qu'est le prochain signe
		\StrBefore\SYS@leftmember\SYS@nextsign[\SYS@currentterm]% prendre ce qu'il y a avant
		\StrBehind\SYS@leftmember\SYS@nextsign[\SYS@leftmember]% et stocker ce qu'il y a ensuite pour apr\`es
		\SYS@assignterm% assigner ce qu'il y a avant avec le dernier signe trouv\'e
		\let\SYS@currentsign\SYS@nextsign% on continue, le prochain signe devient le signe courant
		\expandafter\SYS@spliteqinterms@i\expandafter{\number\numexpr#1+1\expandafter}%
	\fi
}

\SYS@newmacro\SYS@assignterm{%
	\expandafter\SYS@findletter\expandafter{\SYS@currentterm}% trouver le nom de la variable
	\ifx\SYS@letterfound\@empty
		\SYS@consttermtrue
		\ifcsname SYS@term@const@\SYS@eqnumber\endcsname% si terme constant d\'ej\`a rencontr\'e, l'ajouter \`a celui qui existe
			\SYS@expaddtocs\SYS@currentsign\SYS@currentterm
			\expandafter\SYS@expaddtocs\csname SYS@term@const@\SYS@eqnumber\endcsname{\SYS@currentsign}%
		\else
			\SYS@cslet{SYS@sign@const@\SYS@eqnumber}\SYS@currentsign% sinon proc\'eder aux assignations
			\SYS@cslet{SYS@term@const@\SYS@eqnumber}\SYS@currentterm
		\fi
	\else
		\ifcsname SYS@term@\detokenize\expandafter{\SYS@letterfound}@\SYS@eqnumber\endcsname
			\errmessage{Package systeme Error: l'inconnue "\detokenize\expandafter{\SYS@letterfound}" a deja ete trouvee dans l'equation !}%
		\fi
		\ifSYS@sortvariable
			\SYS@insletter\SYS@letterfound% l'ins\'erer si besoin dans la liste ordonn\'ee des variables
		\fi
% 		\show\SYS@letterlist
		\SYS@cslet{SYS@sign@\detokenize\expandafter{\SYS@letterfound}@\SYS@eqnumber}\SYS@currentsign% proc\'eder aux assignations
		\SYS@cslet{SYS@term@\detokenize\expandafter{\SYS@letterfound}@\SYS@eqnumber}\SYS@currentterm
	\fi
}

% cherche la premi\`ere lettre minuscule dans #1
\SYS@newmacro\SYS@findletter#1{%
	\saveexploremode\exploregroups
	\StrRemoveBraces{#1}[\SYS@currentfindletter]%
	\let\SYS@letterfound\@empty
	\SYS@findletter@i
	\restoreexploremode
}

\SYS@newmacro\SYS@findletter@i{%
	\StrSplit\SYS@currentfindletter\@ne\SYS@currentchar\SYS@currentfindletter
	\ifSYS@sortvariable% si le tri auto est activ\'e
		\ifcat\relax\expandafter\noexpand\SYS@currentchar
			\let\SYS@nextaction\@secondoftwo% faux si c'est une sc
		\else
			\ifnum\expandafter`\SYS@currentchar<`a
				\let\SYS@nextaction\@secondoftwo% pas une lettre minuscule
			\else
				\ifnum\expandafter`\SYS@currentchar>`z
					\let\SYS@nextaction\@secondoftwo% pas une lettre minuscule
				\else
					\SYS@testsubscript% tester s'il y a un indice
					\let\SYS@nextaction\@firstoftwo
				\fi
			\fi
		\fi
	\else
		\noexploregroups
		\IfSubStr\SYS@letterlist\SYS@currentchar% ce qui est trouv\'e est dans la liste ?
			{\SYS@testsubscript% tester s'il y a un indice apr\`es le caract\`ere courant
			\let\SYS@nextaction\@firstoftwo
			}%
			{\let\SYS@nextaction\@secondoftwo}%
		\exploregroups
	\fi
	\SYS@nextaction
		{\let\SYS@letterfound\SYS@currentchar
		\IfSubStr\SYS@letterfound_\relax{\SYS@addtocs\SYS@letterfound{_{-1}}}%
		}%
		{\unless\ifx\SYS@currentfindletter\@empty\expandafter\SYS@findletter@i\fi}%
}

\SYS@newmacro\SYS@addtocs#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\SYS@newmacro\SYS@expaddtocs#1#2{\expandafter\SYS@addtocs\expandafter#1\expandafter{#2}}

% teste si \SYS@currentfindletter commence par "_" et si oui, rajoute les 2 caract\`eres \`a \SYS@currentchar et les enl\`eve \`a \SYS@currentfindletter
\SYS@newmacro\SYS@testsubscript{%
	\noexploregroups
	\IfBeginWith\SYS@currentfindletter_%
		{%\StrChar\SYS@currentfindletter\tw@[\SYS@currentletterafter]% TODO BUGFIX
		\StrGobbleLeft\SYS@currentfindletter1[\SYS@currentletterafter]%
%		\show\SYS@currentletterafter
		\exploregroups
		\StrRemoveBraces\SYS@currentletterafter[\SYS@currentletterafter]%
		\IfInteger\SYS@currentletterafter
			{\ifnum\SYS@currentletterafter=\m@ne\errmessage{L'indice ne doit pas etre -1.}\fi}%
			{\errmessage{L'indice n'est pas un nombre entier !}}%
		\SYS@expaddtocs\SYS@currentchar{\expandafter_\expandafter{\SYS@currentletterafter}}%
		}\relax
	\exploregroups
}

% ins\`ere l'inconnue dans la sc #1 \`a sa place dans \SYS@letterlist
\SYS@newmacro\SYS@insletter#1{%
	\IfSubStr\SYS@letterlist{#1}%
		\relax
		{\let\SYS@insunknown#1%
		\StrChar{#1}\thr@@[\SYS@insnum]%
		\StrRemoveBraces\SYS@insnum[\SYS@insnum]%
		\StrChar{#1}\@ne[\SYS@currentinsletter]%
		\let\SYS@letterlist@left\@empty
		\let\SYS@letterlist@right\SYS@letterlist
		\SYS@insletter@i}%
}

\SYS@newmacro\SYS@insletter@i{%
	\ifx\SYS@letterlist@right\@empty% l'inconnue viendra \`a la fin de \SYS@letterlist
		\SYS@expaddtocs\SYS@letterlist@left\SYS@insunknown
		\let\SYS@letterlist\SYS@letterlist@left
	\else
		\StrChar\SYS@letterlist@right\@ne[\SYS@currentletter]% la lettre suivante
		\unless\ifnum\expandafter`\SYS@currentinsletter>\expandafter`\SYS@currentletter% est elle la bonne ?
			\let\SYS@letterlist@right@right\SYS@letterlist@right
			\let\SYS@letterlist@right@left\@empty
			\expandafter\expandafter\expandafter\SYS@insletter@ii%
		\else% sinon
			\StrSplit\SYS@letterlist@right\thr@@\SYS@currentletter\SYS@letterlist@right
			\SYS@expaddtocs\SYS@letterlist@left\SYS@currentletter
			\expandafter\expandafter\expandafter\SYS@insletter@i
		\fi
	\fi
}

\SYS@newmacro\SYS@insletter@ii{%
	\ifx\SYS@letterlist@right@right\@empty
		\let\SYS@letterlist\SYS@letterlist@left
		\SYS@expaddtocs\SYS@letterlist\SYS@letterlist@right@left
		\SYS@expaddtocs\SYS@letterlist\SYS@insunknown
	\else
		\StrChar\SYS@letterlist@right@right\@ne[\SYS@currentletter]% la lettre suivante
		\ifnum\expandafter`\SYS@currentinsletter<\expandafter`\SYS@currentletter% est elle une autre ?
			\let\SYS@letterlist\SYS@letterlist@left
			\SYS@expaddtocs\SYS@letterlist\SYS@letterlist@right@left
			\SYS@expaddtocs\SYS@letterlist\SYS@insunknown
			\SYS@expaddtocs\SYS@letterlist\SYS@letterlist@right@right
		\else
			\StrChar\SYS@letterlist@right@right\thr@@[\SYS@currentsubscript]% le prochain indice
			\StrRemoveBraces\SYS@currentsubscript[\SYS@currentsubscript]%
			\unless\ifnum\SYS@insnum>\SYS@currentsubscript% est-il le bon, c'est-\`a-dire trop grand ?
				\let\SYS@letterlist\SYS@letterlist@left
				\SYS@expaddtocs\SYS@letterlist\SYS@letterlist@right@left
				\SYS@expaddtocs\SYS@letterlist\SYS@insunknown
				\SYS@expaddtocs\SYS@letterlist\SYS@letterlist@right@right
			\else
				\StrSplit\SYS@letterlist@right@right\thr@@\SYS@currentletter\SYS@letterlist@right@right
				\SYS@expaddtocs\SYS@letterlist@right@left\SYS@currentletter
				\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\SYS@insletter@ii
			\fi
		\fi
	\fi
}

\SYS@newmacro\SYS@addtotok#1#2{#1\expandafter{\the#1#2}}

\SYS@newmacro\SYS@expaddtotok#1#2{\expandafter\SYS@addtotok\expandafter#1\expandafter{#2}}

\SYS@newmacro\SYS@addtocode{\SYS@addtotok\SYS@systemecode}

\SYS@newmacro\SYS@expaddtocode#1{\expandafter\SYS@addtocode\expandafter{#1}}

% reconstruit le code du tableau qui sera dans le \halign
\SYS@newmacro\SYS@buildsystem#1#2{% #1=no ligne, #2=no inconnue
	\StrSplit\SYS@letterlist@tmp3\SYS@currentvariable\SYS@letterlist@tmp
	\ifcsname SYS@sign@\detokenize\expandafter{\SYS@currentvariable}@#1\endcsname
		\expandafter\expandafter\expandafter\ifx\csname SYS@sign@\detokenize\expandafter{\SYS@currentvariable}@#1\endcsname+% signe + ?
			\ifnum#2=\@ne% premi\`ere variable ?
				\let\SYS@nextaction\@gobble
			\else
				\ifSYS@firstterm% premier terme de l'\'equation ?'
					\let\SYS@nextaction\@gobble
				\else
					\let\SYS@nextaction\@firstofone
				\fi
			\fi
		\else
			\ifnum#2=\@ne
				\expandafter\def\csname SYS@term@\detokenize\expandafter{\SYS@currentvariable}@#1\expandafter\expandafter\expandafter\endcsname
					\expandafter\expandafter\expandafter{%
					\csname SYS@sign@\detokenize\expandafter{\SYS@currentvariable}@#1\expandafter\expandafter\expandafter\endcsname
					\csname SYS@term@\detokenize\expandafter{\SYS@currentvariable}@#1\endcsname}%
				\let\SYS@nextaction\@gobble
			\else
				\let\SYS@nextaction\@firstofone
			\fi
		\fi
		\SYS@nextaction{%
			\SYS@addtocode{{}}%
			\expandafter\SYS@expaddtocode\expandafter{\csname SYS@sign@\detokenize\expandafter{\SYS@currentvariable}@#1\endcsname{}}%
			}%
		\SYS@firsttermfalse
	\fi
	\unless\ifSYS@star
		\unless\ifnum#2=\@ne\SYS@addtocode&\fi
	\fi
	\ifcsname SYS@term@\detokenize\expandafter{\SYS@currentvariable}@#1\endcsname
		\expandafter\SYS@expaddtocode\expandafter{\csname SYS@term@\detokenize\expandafter{\SYS@currentvariable}@#1\endcsname}%
	\fi
	\unless\ifSYS@star\SYS@addtocode&\fi
	\ifnum#2<\SYS@numberofvariable
		\edef\SYS@nextaction{\noexpand\SYS@buildsystem{#1}{\number\numexpr#2+1}}%
		\expandafter\SYS@nextaction
	\else
		\ifSYS@constterm
			\SYS@addtocode{{}}%
			\ifSYS@firstterm\else\expandafter\SYS@expaddtocode\expandafter{\csname SYS@sign@const@#1\endcsname}\fi
			\SYS@addtocode{{}&}%
			\expandafter\SYS@expaddtocode\expandafter{\csname SYS@term@const@#1\endcsname&}%
		\fi
		\ifcsname SYS@eqsign@#1\endcsname
			\SYS@addtocode{{}}%
			\expandafter\SYS@expaddtocode\expandafter{\csname SYS@eqsign@#1\endcsname{}&}%
			\expandafter\SYS@expaddtocode\expandafter{\csname SYS@right@#1\endcsname}%
		\else
			\SYS@addtocode&%
		\fi
		\saveexploremode\exploregroups
		\ifcsname SYS@extracol@#1\endcsname
			\SYS@addtocode&%
			\expandafter\IfSubStr\csname SYS@extracol@#1\endcsname{**}% le contenu de l'extra col contient-il "**" ?
				{\expandafter\let\expandafter\SYS@autonumarg\csname SYS@extracol@#1\endcsname
				\StrSubstitute\SYS@autonumarg{**}{\number\numexpr\SYSeqnum+#1-\SYS@eqnumber}[\SYS@currentautonum]%
				\SYS@cslet{SYS@extracol@#1}\SYS@currentautonum
				\SYS@autonumtrue
				}%
				{\expandafter\IfSubStr\csname SYS@extracol@#1\endcsname*% le contenu de l'extra col contient-il "*" ?
					{\expandafter\let\expandafter\SYS@autonumarg\csname SYS@extracol@#1\endcsname
					\StrSubstitute\SYS@autonumarg*{\noexpand#1}[\SYS@currentautonum]%
					\SYS@cslet{SYS@extracol@#1}\SYS@currentautonum
					\SYS@autonumtrue
					}%
					{\ifSYS@autonum
						\IfSubStr\SYS@autonumarg{**}%
							{\StrSubstitute\SYS@autonumarg{**}{\number\numexpr\SYSeqnum+#1-\SYS@eqnumber}[\SYS@currentautonum]}%
							{\StrSubstitute\SYS@autonumarg*{\noexpand#1}[\SYS@currentautonum]}%
						\SYS@expaddtocode\SYS@currentautonum
					\fi
					}%
				}%
			\expandafter\SYS@expaddtocode\expandafter{\csname SYS@extracol@#1\endcsname}%
		\else% pas d'extra colonne pour cette ligne ?
			\ifSYS@autonum% mais si il y un autonum
				\SYS@addtocode&%
				\IfSubStr\SYS@autonumarg{**}%
					{\StrSubstitute\SYS@autonumarg{**}{\number\numexpr\SYSeqnum+#1-\SYS@eqnumber}[\SYS@currentautonum]}%
					{\StrSubstitute\SYS@autonumarg*{\noexpand#1}[\SYS@currentautonum]}%
				\SYS@expaddtocode\SYS@currentautonum
			\fi
		\fi
		\restoreexploremode
		\ifnum#1<\SYS@eqnumber
			\SYS@addtocode\cr
			\SYS@firsttermtrue
			\let\SYS@letterlist@tmp\SYS@letterlist
			\edef\SYS@nextaction{\noexpand\SYS@buildsystem{\number\numexpr#1+1}{1}}%
			\expandafter\expandafter\expandafter\SYS@nextaction
		\else% fin de l'alignement
			\SYS@addtocode{\SYS@strutdown\cr}%
		\fi
	\fi
}

% ajoute "_\m@ne" \`a tous les tokens de #1 qui n'ont pas un indice
\SYS@newmacro\SYS@scanletterlist#1{%
	\let\SYS@letterlist\@empty
	\def\SYS@lettersremaining{#1}%
	\SYS@scanletterlist@i
}

\SYS@newmacro\SYS@scanletterlist@i{%
	\StrSplit\SYS@lettersremaining\@ne\SYS@currentchar\SYS@lettersremaining
	\SYS@expaddtocs\SYS@letterlist\SYS@currentchar
	\IfBeginWith\SYS@lettersremaining_%
		{\StrChar\SYS@lettersremaining\tw@[\SYS@currentchar]%
		\StrRemoveBraces\SYS@currentchar[\SYS@currentchar]%
		\SYS@expaddtocs\SYS@letterlist{\expandafter_\expandafter{\SYS@currentchar}}%
		\StrGobbleLeft\SYS@lettersremaining\tw@[\SYS@lettersremaining]%
		}%
		{\SYS@addtocs\SYS@letterlist{_{-1}}}%
	\unless\ifx\SYS@lettersremaining\empty\expandafter\SYS@scanletterlist@i\fi
}

\SYS@newmacro\sysdelim#1#2{\def\SYS@delim@left{\left#1}\def\SYS@delim@right{\right#2}}
\sysdelim\{.

\SYS@newmacro\systeme{\@ifstar{\SYS@startrue\SYS@systeme@i}{\SYS@starfalse\SYS@systeme@i}}

\SYS@newmacro\SYS@systeme@i{%
	\relax\iffalse{\fi\ifnum0=`}\fi
	\begingroup
		\mathcode`\,="013B
		\catcode`\^7 \catcode`\_8
		\expandarg\noexploregroups
		\setbox\z@\hbox{$($}%
		\edef\SYS@strutup{\vrule depth\z@ width\z@ height\dimexpr\ht\z@+\SYS@extrastrutdim\relax}%
		\edef\SYS@strutdown{\vrule height\z@ width\z@ depth\dimexpr\dp\z@+\SYS@extrastrutdim\relax}%
		\SYS@cslet++\SYS@cslet--%
		\@testopt\SYS@systeme@ii{}%
}

\SYS@newmacro\SYS@systeme@ii[#1]{%
		\ifx\@empty#1\@empty
			\let\SYS@letterlist\@empty
			\SYS@sortvariabletrue
		\else
			\SYS@scanletterlist{#1}% ajoute des _{-1} si besoin
			\SYS@sortvariablefalse
		\fi
		\SYS@consttermfalse
		\expandafter\@testopt\expandafter\SYS@systeme@iii\expandafter{\SYS@defaulteqsep}%
}

\SYS@newmacro\SYS@systeme@iii[#1]#2{%
		\SYS@newmacro\SYS@systeme@iv##1#1##2\@nil{%
			\ifx\@empty##1\@empty
				\SYS@addtocode\cr% une ligne vide
			\else
				\SYS@spliteqinterms{##1}% analyser l'eq courante
			\fi
			\ifx\@empty##2\@empty% tant qu'il reste des \'equations
			\else
				\edef\SYS@eqnumber{\number\numexpr\SYS@eqnumber+\@ne}% augmenter de 1 leur nombre
				\global\advance\SYSeqnum\@ne
				\def\SYS@nextaction{\SYS@systeme@iv##2\@nil}% recommencer avec ce qu'il reste
				\expandafter\SYS@nextaction
			\fi
		}%
		\global\advance\SYSeqnum\@ne
		\def\SYS@eqnumber{1}%
		\ifdefined\SYS@autonumarg
			\ifx\SYS@autonumarg\@empty% on initialise que si \SYS@autonumarg est vide
				\SYS@extracolfalse
				\SYS@autonumfalse
			\fi
		\else
			\SYS@extracolfalse
			\SYS@autonumfalse
		\fi
		\SYS@systeme@iv#2#1\@nil% analyser toutes les \'equations et en faire des termes et des signes
		\StrCount\SYS@letterlist_[\SYS@numberofvariable]%
		\SYS@systemecode{}\SYS@systempreamble{}%
		\ifSYS@star
			\SYS@makesyspreamble\@ne
		\else
			\SYS@makesyspreamble\SYS@numberofvariable% fabriquer le pr\'eambule du \halign
		\fi
		\SYS@firsttermtrue
		\let\SYS@letterlist@tmp\SYS@letterlist
		\SYS@buildsystem11% construire le syst\`eme...
		\ifdefined\SYS@substlist
			\unless\ifx\SYS@substlist\@empty
				\edef\SYS@systemcs{\the\SYS@systemecode}%
				\SYS@substlist
				\SYS@systemecode\expandafter{\SYS@systemcs}%
			\fi
		\fi
		\ifmmode
			\expandafter\@firstofone
		\else
			\expandafter\SYS@entermath
		\fi
			{\SYS@delim@left
			\vcenter{%
				\lineskiplimit\z@\lineskip\z@
				\baselineskip\SYS@lineskipcoeff\normalbaselineskip
				\halign\expandafter\expandafter\expandafter{\expandafter\the\expandafter\SYS@systempreamble\the\SYS@systemecode}%
				}%
			\SYS@delim@right
			}% ...l'afficher en mode math
	\endgroup
	\ifnum0=`{\fi\iffalse}\fi
	\unless\ifSYS@followautonum
		\ifdefined\SYS@autonumarg
			\let\SYS@autonumarg\@empty% annule la num\'erotation auto
		\fi
	\fi
}

% Construire le pr\'eambule du \halign
\SYS@newmacro\SYS@makesyspreamble#1{%
	\def\SYS@preamblenum{#1}%
	\SYS@makesyspreamble@i\@ne
}

\SYS@newmacro\SYS@makesyspreamble@i#1{%
	\ifnum#1<\SYS@preamblenum% tant qu'il reste des variables
		\SYS@addtotok\SYS@systempreamble{\hfil$##$&\hfil$##$&}% une colonne pour le terme et une pour le signe
		\expandafter\SYS@makesyspreamble@i\expandafter{\number\numexpr#1+\@ne\expandafter}%
	\else
		\ifSYS@constterm
			\SYS@addtotok\SYS@systempreamble{\hfil$##$&\hfil$##$&}% une colonne pour le terme constant et son signe
		\fi
		\SYS@addtotok\SYS@systempreamble{\hfil$##$&$##$&$##$\hfil\null}% ajouter 1 colonne pour le signe = et une pour le terme de droite
		\ifSYS@extracol
			\SYS@addtotok\SYS@systempreamble{&\SYS@extracolstart##\SYS@extracolend\hfil\null}% la colonne suppl\'ementaire (pas de mode math)
		\fi
		\SYS@addtotok\SYS@systempreamble{\cr\SYS@strutup}% ajouter la fin du pr\'eambule et le strut de premi\`ere ligne
	\fi
}

\SYS@newmacro\SYS@entermath#1{$\relax#1$}

% d\'efinit les substitutions \`a faire dans le tableau avant l'affichage
\SYS@newmacro\syssubstitute{%
	\unless\ifdefined\SYS@substlist\let\SYS@substlist\@empty\fi
	\SYS@substitute@i
}

\SYS@newmacro\SYS@substitute@i#1{%
	\ifx\@empty#1\@empty
	\else
		\SYS@addtocs\SYS@substlist{\StrSubstitute\SYS@systemcs}%
		\StrChar{\noexpand#1}\@ne[\SYS@currentchar]\StrRemoveBraces\SYS@currentchar[\SYS@currentchar]%
		\SYS@expaddtocs\SYS@substlist{\expandafter{\expandafter\noexpand\SYS@currentchar}}%
		\StrChar{\noexpand#1}\tw@[\SYS@currentchar]\StrRemoveBraces\SYS@currentchar[\SYS@currentchar]%
		\SYS@expaddtocs\SYS@substlist{\expandafter{\expandafter\noexpand\SYS@currentchar}[\SYS@systemcs]}%
		\def\SYS@nextaction{\expandafter\SYS@substitute@i\expandafter{\@gobbletwo#1}}%
		\expandafter\SYS@nextaction
	\fi
}

% annule les substitutions
\SYS@newmacro\sysnosubstitute{\let\SYS@substlist\@empty}

\catcode`\@\SYS@savedatcatcode\relax

\endinput

######################################################################
#                             Historique                             #
######################################################################

v0.1        27/02/2011
	- Premi\`ere version publique sur le CTAN
----------------------------------------------------------------------
v0.2        08/03/2011
    - Le premier argument optionnel met en place de nouvelles
      fonctionnalit\'es
    - Possibilit\'e d'avoir des inconnues indic\'ees
    - Mise en place d'une colonne suppl\'ementaire et d'une
      num\'erotation automatique
    - La commande \'etoil\'ee \systeme* d\'egrade l'alignement pour ne
      plus prendre en compte que les signes d'\'egalit\'e
    - Une substitution est possible en fin de traitement, juste
      avant d'afficher le syst\`eme.
----------------------------------------------------------------------
v0.2a       15/05/2011
    - Bug corrig\'e lorsque les termes comportent des accolades
----------------------------------------------------------------------
v0.2b       2011/06/23
    - La commande \setdelim permet de modifier les d\'elimiteurs
      extensibles plac\'es de part et d'autre du syst\`eme.
----------------------------------------------------------------------
v0.3        21/12/2013
    - Un terme constant est permis dans le membre de gauche
    ----------------------------------------------------------------------
v0.31       01/01/2018
    - Il manquait un "&" apr\`es le terme constant, merci \`a Thomas Soll
      de l'avoir signal\'e

==> xstring.tex <==
%  __________________________________________________
% |                                                  |
% |                                                  |
% |                   xstring v1.7c                  |
% |                                                  |
% |                  13 octobre 2013                 |
% |                                                  |
% |__________________________________________________|
%
% This is xtring.tex
%
% "xstring" package consists of the 7 following files:
%   xstring.tex (this file)
%   xstring.sty
%   README
%   xstring_doc_fr.tex, xstring_doc_fr.pdf (manual in french)
%   xstring_doc_en.tex, xstring_doc_en.pdf (manual in english)
%
% Christian Tellechea 2008-2013
% email : unbonpetit@gmail.com
% -------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
%     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% -------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% -------------------------------------------------------------------
\def\xstringversion     {1.7c}
\def\xstringdate        {2013/10/13}
\def\xstringfrenchdate  {13 octobre 2013}
\def\xstringenglishdate {13 october 2013}
\edef\CurrentAtCatcode  {\the\catcode`\@}
\catcode`\@=11
\newwrite\@xs@message% canal pour les messages
\newcount\integerpart
\newcount\decimalpart% compteurs utilis\'es par xstring

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\immediate\write\m@ne{Package: xstring \xstringdate\space\space v\xstringversion\space\space String manipulations}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@gobble#1{}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
\fi% fin des d\'efinitions LaTeX

\long\def\@xs@ifempty#1{%
	\expandafter\ifx\expandafter\relax\detokenize{#1}\relax
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}
% Ouvre un groupe o\`u les catcodes sont \`a 12 et \`a 10 pour les espaces
% ensuite, appelle \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\@xs@MakeVerb{% lit 1 argument et le transforme en verb
	\begingroup% groupe o\`u les catcodes sont \`a 12 pour la lecture suivante
		\def\do##1{\catcode`##112\relax}%
		\dospecials% on entre dans le mode verb
		\obeyspaces% et on tient compte des espaces
		\@xs@ReadVerb% et on va lire l'argument
}

% D\'efinit \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\setverbdelim#1{% d\'efinit quel est le d\'elimiteur de verb
	\expandafter\@xs@ifempty\expandafter{\@gobble#1}%
		\relax
		{\begingroup
			\newlinechar`\^^J%
			\immediate\write\@xs@message
			{Package xstring Warning: verb delimiter is not a single token on input line \the\inputlineno^^J}%
		\endgroup
		}%
	\def\@xs@ReadVerb##1#1##2#1{% lit ##2 qui est entre les d\'elimiteurs de verb
		\endgroup% on ferme le groupe
		\@xs@afterreadverb{##2}}% on appelle l'ex\'ecution de fin
}

% Assigne l'argument entre d\'elimiteur verb dans la sc #1' +
\def\verbtocs#1{%
	\def\@xs@afterreadverb##1{\def#1{##1}}%
	\@xs@MakeVerb
}

\begingroup
	\catcode\z@3 \def\@xs@twochars{^^00}%
	\catcode\z@7 \xdef\@xs@twochars{\@xs@twochars^^00}%
\endgroup

\edef\@xs@reserved@A{\long\def\noexpand\@xs@AssignResult##1\@xs@twochars}

\@xs@reserved@A#2{\endgroup\expandafter\def\expandafter#2\expandafter{\@gobble#1}}

\def\tokenize#1#2{%
	\begingroup
		\@xs@def\@xs@reserved@A{#2}% on d\'eveloppe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\@xs@twochars#1}% met "^^@^^@#1" \`a la fin du fichier virtuel
		\endlinechar\m@ne
		\expandafter\@xs@AssignResult\scantokens\expandafter{\expandafter\relax\@xs@reserved@A}% on fait l'assignation
}%

% Macro tr\`es simple qui assigne ou affiche le r\'esultat, selon la pr\'esence
% ou non de #2 qui est l'argument optionnel venant en derni\`ere position des macros
\long\def\@xs@ReturnResult#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#2}%
		\@xs@argument@A
		{\let#2\@xs@argument@A}%
}

\def\@xs@ldef{\long\def}

\def\@xs@ledef{\long\edef}

% Pas d'expansion des arguments
\def\normalexpandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter{##1}}}
\let\noexpandarg\normalexpandarg% synonyme

% 1-d\'eveloppement du premier token des arguments
\def\expandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

% D\'eveloppement maximum des arguments
\def\fullexpandarg{%
	\let\@xs@def\@xs@ledef% on d\'efinit\@xs@call avec \edef
	\def\@xs@expand##1{##1}% et on neutralise \@xs@expand
}

\def\saveexpandmode{\let\@xs@saved@def\@xs@defarg\let\@xs@saved@expand\@xs@expand}

\def\restoreexpandmode{\let\@xs@defarg\@xs@saved@def\let\@xs@expand\@xs@saved@expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\@xs@ifbeginwithbrace#1{%
	\csname @%
		\expandafter\@gobble\string{%
		\expandafter\@gobble\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@firstoftwo
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\@gobble\string}%
		\@secondoftwo{first}{second}oftwo%
	\endcsname
}

% Cette macro interne prend la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@returnfirstsyntaxunit#1#2{%
	\def\@xs@groupfound{\expandafter\def\expandafter#2\expandafter{\expandafter{#2}}\@xs@gobbleall}% on met #2 dans des accolades et on finit
	\long\def\@xs@assignfirsttok##1##2\@xs@nil{\let\@xs@toks0\def#2{##1}}%
	\def\@xs@testfirsttok{%
		\let\@xs@next\@xs@assignfirsttok
		\ifx\@xs@toks\bgroup
			\expandafter\@xs@ifbeginwithbrace\expandafter{\@xs@argument}{\def\@xs@next{\afterassignment\@xs@groupfound\def#2}}{}%
		\fi
		\@xs@next}%
	\def\@xs@argument{#1}%
	\edef\@xs@next{\expandafter\@xs@beforespace\detokenize{#1} \@xs@nil}% #1 commence par un espace ?
	\ifx\@xs@next\@empty
		\def\@xs@next{\expandafter\ifx\expandafter\@empty\detokenize\expandafter{\@xs@argument}\@empty\let#2\@empty\else\def#2{ }\let\@xs@toks0\fi}%
	\else
		\def\@xs@next{\expandafter\futurelet\expandafter\@xs@toks\expandafter\@xs@testfirsttok\@xs@argument\@xs@nil}%
	\fi
	\@xs@next
}

% Cette macro interne enl\`eve la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@testsecondtoken#1\@xs@nil{\@xs@ifbeginwithbrace{#1}}

\long\def\@xs@gobblespacebeforebrace#1#{}% supprime tout ce qui est avant la 1ere accolade ouvrante

\long\def\@xs@removefirstsyntaxunit#1#2{%
	\def\@xs@argument{#1}%
	\expandafter\expandafter\expandafter\ifx\expandafter\expandafter\expandafter\@empty\expandafter\@xs@beforespace\detokenize\expandafter{\@xs@argument} \@xs@nil\@empty% #1 commence par un espace ?
		\expandafter\@xs@ifempty\expandafter{\@xs@argument}%
			{\let#2\@empty}
			{\afterassignment\@xs@testsecondtoken% après avoir mangé le 1er token, on va tester si la suite commence par «{»
			\expandafter\let\expandafter\@xs@secontoken\expandafter=\expandafter\@sptoken\@xs@argument\@xs@@nil\@xs@nil% on mange le 1er token et on rajoute \@xs@@nil à la fin pour éviter de perdre les accolades du groupe
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@gobblespacebeforebrace\@xs@argument}}%
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@behindspace\@xs@argument\@xs@nil}}%
			}%
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
		\expandafter\expandafter\expandafter{\expandafter\@gobble\@xs@argument}%
	\fi
}

% Macros \`a arguments d\'elimit\'es pour les macros ci dessus
\long\def\@xs@beforespace#1 #2\@xs@nil{#1}

\long\def\@xs@behindspace#1 #2\@xs@nil{#2}

\long\def\@xs@returnfirstsyntaxunit@ii#1#2\@xs@nil{#1}

\long\def\@xs@gobbleall#1\@xs@nil{}

% Cette macro interne est utilis\'ee dans les macros \'etoil\'ees pour :
% 1) d\'evelopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci \`a l'aide de la macro \@xs@def
% 2) Ensuite, on d\'etokenize ce d\'eveloppement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\@xs@expand@and@detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\@xs@expand#1}% on d\'eveloppe #2 selon le mode de d\'eveloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d\'etokenize et on assigne \`a #1
}

\long\def\@xs@expand@and@assign#1#2{\@xs@def#1{#2}}% on d\'eveloppe #2 selon \fullexpandarg ou \normalexpandarg

\long\def\@xs@edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}

\long\def\@xs@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\def\@xs@argstring{0########1########2########3########4########5########6########7########8########9}

% \@xs@DefArg{3} met dans la sc \@xs@myarg les tokens "####1####2####3"
\def\@xs@DefArg#1{\def\@xs@defarg0##1#1##2\@xs@nil{\def\@xs@myarg{##1#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@DefArg@{3} met dans la sc \@xs@myarg les tokens "[####1]####2####3####4"
\def\@xs@DefArg@#1{\expandafter\@xs@defarg@\expandafter{\number\numexpr#1+1}}

\def\@xs@defarg@#1{\def\@xs@defarg0##11##2#1##3\@xs@nil{\def\@xs@myarg{[##11]##2#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@OneArg{3} met dans la sc \@xs@myarg les tokens "####3"
\def\@xs@OneArg#1{\expandafter\@xs@onearg\expandafter{\number\numexpr#1-1}{#1}}

\def\@xs@onearg#1#2{\def\@xs@defarg##1#1##2#2##3\@xs@nil{\def\@xs@myarg{##2#2}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% #1 : num\'ero du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num\'ero de l'argument devant être d\'etokenis\'e si \'etoile
\def\@xs@BuildLines#1#2#3#4{%
	\let\@xs@newlines\@empty
	\let\@xs@newargs\@empty
	\def\@xs@buildlines##1{%
		\expandafter\@xs@OneArg\expandafter{\number\numexpr##1+#1-1}%
		\edef\@xs@reserved@B{\noexpand\@xs@expand\csname @xs@arg@\romannumeral\numexpr##1\endcsname}%
		\ifnum##1=\@ne% si c'est le premier argument
			\@xs@ifempty{#3}%
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
				\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter[\@xs@reserved@B]}%
				\def\@xs@reserved@B{@xs@def}% ne pas d\'etok\'eniser l'argument optionnel grace au \@xs@def
				}
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
			\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
		\fi
		\edef\@xs@newlines{\unexpanded\expandafter{\@xs@newlines}\expandafter\noexpand\csname\@xs@reserved@B\endcsname\expandafter\noexpand\csname @xs@arg@\romannumeral\numexpr##1\endcsname{\@xs@myarg}}%
		\ifnum##1<#2\relax
			\def\@xs@next{\expandafter\@xs@buildlines\expandafter{\number\numexpr##1+1}}%
			\expandafter\@xs@next
		\fi}%
	\@xs@buildlines\@ne
}

\def\@xs@newmacro{%
	\@ifstar
		{\let\@xs@reserved@D\@empty\@xs@newmacro@}
		{\let\@xs@reserved@D\relax\@xs@newmacro@0}%
}

% #1 : dernier num\'ero de l'argument devant être d\'etokenis\'e
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\@xs@newmacro@#1#2#3#4#5{%
	\edef\@xs@reserved@A{@xs@\expandafter\@gobble\string#2}%
	\edef\@xs@reserved@C{\expandafter\noexpand\csname\@xs@reserved@A @\ifx\@empty#3\@empty @\fi\endcsname}%
	\edef\@xs@reserved@B{%
		\ifx\@empty\@xs@reserved@D
			\def\noexpand#2{\noexpand\@ifstar
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@detokenize\expandafter\noexpand\@xs@reserved@C}%
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
		\fi
		\ifx\@empty#3\@empty
		\else
			\def\expandafter\noexpand\@xs@reserved@C{%
				\noexpand\@testopt{\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname}{\ifx\@xs@def\@xs@ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit :
	% si #3 est vide : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@@}}
	% si #3 existe   : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@}}
	%                  \@xs@NOM@{\@testopt{\@xs@NOM@@}{#3}}}
	\long\@xs@reserved@B
	\ifx\@empty#3\@empty
		\@xs@BuildLines1{#4}{#3}{#1}%
		\@xs@DefArg{#4}%
	\else
		\expandafter\@xs@BuildLines\expandafter1\expandafter{\number\numexpr#4+1}{#3}{#1}%
		\@xs@DefArg@{#4}%
	\fi
	\edef\@xs@reserved@B{\def\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname\@xs@myarg}%
	\edef\@xs@reserved@C{\unexpanded\expandafter{\@xs@newlines}\edef\noexpand\@xs@call}%
	\edef\@xs@reserved@D{%
		\noexpand\noexpand\expandafter\noexpand\csname\@xs@reserved@A\endcsname\unexpanded\expandafter{\@xs@newargs}%
	}%
	\ifnum#5=\@ne\edef\@xs@reserved@D{\noexpand\noexpand\noexpand\@testopt{\unexpanded\expandafter{\@xs@reserved@D}}{}}\fi
	\@xs@edefaddtomacro\@xs@reserved@C{{\unexpanded\expandafter{\@xs@reserved@D}}\noexpand\@xs@call}%
	\@xs@edefaddtomacro\@xs@reserved@B{{\unexpanded\expandafter{\@xs@reserved@C}}}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\@xs@NOM@@[##2]##3##4##5{%
	%          \@xs@def\@xs@arg@i{##2}\@xs@assign\@xs@arg@ii{##3}\@xs@assign\@xs@arg@iii{##4}\@xs@asign\@xs@arg@iv{##5}%
	% si #5=0: \edef\@xs@call{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}%
	% si #5=1: \edef\@xs@call{\noexpand\@testopt{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@i}{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}{}}%
	%          \@xs@call}
	\long\@xs@reserved@B
	\edef\@xs@reserved@B{%
		\def\expandafter\noexpand\csname\@xs@reserved@A\endcsname
			\@xs@myarg\ifnum#5=\@ne[\unexpanded{##}\number\numexpr\ifx\@empty#3\@empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \@xs@NOM[##2]##3##4##5[##6]{#6}
	\long\@xs@reserved@B
}

% macro g\'en\'erique qui lit \@xs@reserved@C us par us
% 3 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atbegingroup      (un groupe vient d'être ouvert)
% \@xs@atnextsyntaxunit  (la future US n'est pas un groupe)
\def\@xs@read@reserved@C{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@read@reserved@C
		\@xs@exploregroups
		\ifx\bgroup\@xs@toks
			\advance\integerpart\@ne
			\begingroup
				\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
				\@xs@manage@groupID
				\let\@xs@nestlevel\@ne
				\integerpart\z@
				\@xs@atbegingroup
		\else
			\global\advance\decimalpart\@ne
			\@xs@atnextsyntaxunit
		\fi
		}%
	\@xs@next
}

% macro g\'en\'erique qui lit \@xs@reserved@D en proc\'edant \`a des tests avec \IfBeginWith
% 2 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atoccurfound      (une occurrence a \'et\'e trouv\'ee)
\def\@xs@read@reserved@D{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}%
		{\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
			{\expandafter\@xs@reserved@D\expandafter}\expandafter{\@xs@reserved@E}%
			{\global\advance\decimalpart\@ne
			\let\@xs@reserved@D\@xs@reserved@A
			\@xs@atoccurfound
			}%
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@A
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
			\let\@xs@next\@xs@read@reserved@D
			\@xs@exploregroups
			\ifx\bgroup\@xs@toks
				\advance\integerpart\@ne
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@D\@xs@reserved@A
					\@xs@manage@groupID
					\let\@xs@reserved@C\@empty
					\let\@xs@nestlevel\@ne
					\integerpart\z@
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro\StrRemoveBraces{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\let\@xs@reserved@B\@empty
	\let\@xs@nestlevel\z@
	\@xs@StrRemoveBraces@i
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#2}%
}

\def\@xs@StrRemoveBraces@i{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@B}%
			\let\@xs@next\@xs@StrRemoveBraces@i
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@StrRemoveBraces@i
		\ifx\bgroup\@xs@toks
			\ifx\@xs@exploregroups\relax% on explore les groupes ?
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
					\let\@xs@nestlevel\@ne
					\integerpart\z@
					\let\@xs@reserved@B\@empty
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\@xs@reserved@A
			\fi
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
		\fi
		}%
	\@xs@next
}

% \@xs@cutafteroccur coupe l'argument #1 apr\`es la #3\`eme occurrence de #2
% \@xs@reserved@C : contient ce qui se trouve avant cette occurrence
% \@xs@reserved@D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \@xs@reserved@E : contient ce qui se trouve apr\`es l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy\'ees sont vides
\long\def\@xs@cutafteroccur#1#2#3{%
	\ifnum#3<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
		}
		{\@xs@cutafteroccur@i{#1}{#2}{#3}}%
}
	
\long\def\@xs@cutafteroccur@i#1#2#3{%
	\def\@xs@reserved@D{#1}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#2}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\ifnum\decimalpart=\numexpr(#3)\relax % occurrence trouv\'ee ?
		\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\@xs@argument@A}%
	\else
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
	\fi
}

\@xs@newmacro*3\IfSubStr{1}{2}{0}{%
	\def\@xs@argument@A{#2}\def\@xs@argument@B{#3}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur
	\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter{\@xs@argument@B}{#1}%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*2\IfBeginWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@secondoftwo
		}
		{\def\@xs@next{%
			\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
				{\expandafter\@xs@argument@A\expandafter}\expandafter
				{\@xs@argument@B}}%
		}%
	\@xs@next
}

\long\def\@xs@IfBeginWith@i#1#2{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@firstoftwo% #2 est vide, tous les tests sont pass\'es avec succ\`es : on renvoie #3
		}
		{\expandafter\@xs@ifempty\expandafter{\@xs@argument@A}%
			{\let\@xs@next\@secondoftwo% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
			\ifx\@xs@reserved@A\@xs@reserved@B% il y a \'egalit\'e...
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A% on enl\`eve les 1ere unit\'es syntaxiques
				\def\@xs@next{% et on recommence avec ces arguments racourcis d'1 unit\'e syntaxique
					\expandafter\expandafter\expandafter\@xs@IfBeginWith@i
					\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}}%
			\else
				\let\@xs@next\@secondoftwo
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro*2\IfEndWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\@xs@ifempty{#2}%
		{\let\@xs@reserved@A\@secondoftwo
		}
		{\expandafter\expandafter\expandafter\@xs@StrCount
			\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter
			{\@xs@argument@B}[\@xs@reserved@A]%
		\ifnum\@xs@reserved@A=\z@
			\let\@xs@reserved@A\@secondoftwo
		\else
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
				{\let\@xs@reserved@A\@firstoftwo}
				{\let\@xs@reserved@A\@secondoftwo}%
		\fi
		}%
	\@xs@reserved@A
}

\@xs@newmacro*4\IfSubStrBefore{1,1}{3}{0}{\@xs@IfSubStrBefore@i[#1]{#2}{#3}{#4}}

\def\@xs@IfSubStrBefore@i[#1,#2]#3#4#5{%
	\def\@xs@reserved@C{#3}%
	\ifx\@xs@exploregroups\relax% si on explore les groupes
		\let\@xs@reserved@B\@empty
		\let\@xs@nestlevel\z@
		\@xs@StrRemoveBraces@i% on retire les accolades
		\let\@xs@reserved@C\@xs@reserved@B
	\fi
	\def\@xs@reserved@A{#5}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#2}%
	\def\@xs@reserved@A{#4}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#1}%
	\global\let\groupID\@empty
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*4\IfSubStrBehind{1,1}{3}{0}{\@xs@IfSubStrBehind@i[#1]{#2}{#3}{#4}}

\long\def\@xs@IfSubStrBehind@i[#1,#2]#3#4#5{\@xs@IfSubStrBefore@i[#2,#1]{#3}{#5}{#4}}

\long\def\@xs@formatnumber#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\@xs@returnfirstsyntaxunit{#1}\@xs@reserved@A
		\def\@xs@reserved@B{+}%
		\ifx\@xs@reserved@A\@xs@reserved@B
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@C
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			 	{\def#2{+0X}}
			 	{\expandafter\def\expandafter#2\expandafter{\expandafter+\expandafter0\@xs@reserved@C}}%
		\else
			\def\@xs@reserved@B{-}%
			\ifx\@xs@reserved@A\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
				\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
					{\def#2{-0X}}%
					{\expandafter\def\expandafter#2\expandafter{\expandafter-\expandafter0\@xs@reserved@A}}%
			\else
				\expandafter\def\expandafter#2\expandafter{\expandafter0\@xs@argument@A}%
			\fi
		\fi
		}%
}

\@xs@newmacro\IfInteger{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\let\@xs@after@intpart\@xs@afterinteger
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\ifnum\decimalpart=\z@
			\let\@xs@next\@firstoftwo% partie décimale constituée de 0 --> seul cas où on renvoie vrai
		\else
			\let\@xs@afterinteger\@xs@after@intpart
			\let\@xs@next\@secondoftwo
		\fi
	\else
		\let\@xs@afterinteger\@xs@after@intpart
		\let\@xs@next\@secondoftwo
	\fi
	\@xs@next
}

\@xs@newmacro\IfDecimal{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}

\long\def\@xs@defafterinteger#1\relax\@xs@nil{\def\@xs@afterinteger{#1}}

\def\@xs@testdot{%
	\let\xs@decsep\@empty
	\@ifnextchar.%
		{\def\xs@decsep{.}\@xs@readdecimalpart}%
		{\@xs@testcomma}%
}

\def\@xs@testcomma{%
	\@ifnextchar,%
		{\def\xs@dessep{,}\@xs@readdecimalpart}%
		{\@xs@endnumber}%
}

\long\def\@xs@readdecimalpart#1#2\@xs@nil{%
	\ifx\@empty#2\@empty
		\def\@xs@reserved@A{0X}%
	\else
		\def\@xs@reserved@A{0#2}%
	\fi
	\afterassignment\@xs@defafterinteger\decimalpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@endnumber\@xs@afterinteger\@xs@nil
}

\long\def\@xs@endnumber#1\@xs@nil{\def\@xs@afterdecimal{#1}}

% test d'\'egalit\'e sur des chaines (et des chaines contenant des nombres)
\long\def\@xs@IfStrEqFalse@i#1#2{\let\@xs@reserved@A\@secondoftwo}
\long\def\@xs@IfStrEqFalse@ii#1#2{% renvoie vrai si les 2 arg sont d\'ecimaux et s'ils sont \'egaux, faux sinon
	\@xs@IfDecimal{#1}%
		{\@xs@IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\@xs@reserved@A\@firstoftwo
			\else
				\let\@xs@reserved@A\@secondoftwo
			\fi% les 2 sont d\'ecimaux : on fait le test
			}%
			{\let\@xs@reserved@A\@secondoftwo}% un seul est d\'ecimal
		}%
		{\let\@xs@reserved@A\@secondoftwo}% #1 n'est pas d\'ecimal
}

\long\def\@xs@TestEqual#1#2{% teste si les 2 arguments sont \'egaux
	\def\@xs@reserved@A{#1}\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\let\@xs@reserved@A\@firstoftwo% \'egalit\'e parfaite des 2 chaines
	\else
		\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}%
	\fi
	\@xs@reserved@A
}

\@xs@newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont \'egales
	\let\@xs@reserved@D\@xs@IfStrEqFalse@i
	\@xs@TestEqual{#1}{#2}%
}

\@xs@newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont \'egaux
	\let\@xs@reserved@D\@xs@IfStrEqFalse@ii
	\@xs@TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfStrEq*}\@xs@IfStrCase}%
		{\def\@xs@reserved@E{\IfStrEq}\@xs@IfStrCase}%
}

\long\def\@xs@IfStrCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\def\IfEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfEq*}\@xs@IfEqCase}%
		{\def\@xs@reserved@E{\IfEq}\@xs@IfEqCase}%
}

\long\def\@xs@IfEqCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\long\def\@xs@IfStringCase#1#2[#3]{%
	\long\def\@xs@testcase##1##2##3\@xs@nil{% lit les 2 premieres unit\'es syntaxiques dans ##1 et ##2. Les autres dans ##3
		\@xs@reserved@E{#1}{##1}%
			{##2}% le test est positif, on ex\'ecute le code correspondant
			{\@xs@ifempty{##3}%
			 	{#3}% s'il n'y a plus de cas, on ex\'ecute le code <autres cas>
				{\@xs@testcase##3\@xs@nil}% sinon, on recommence avec ce qui reste
			 }%
	}%
	\@xs@testcase#2\@xs@nil
}

% Renvoie ce qui est \`a gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBefore{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
}

% Renvoie ce qui est \`a droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBehind{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\@xs@newmacro*4\StrBetween{1,1}{3}{1}{\@xs@StrBetween@i[#1]{#2}{#3}{#4}[#5]}

\long\def\@xs@StrBetween@i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\@xs@cutafteroccur{#3}{#5}{#2}%
		\expandafter\@xs@cutafteroccur\expandafter{\@xs@reserved@C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#6}%
	\global\let\groupID\@empty
}

\def\exploregroups{\let\@xs@exploregroups\relax}

\def\noexploregroups{\def\@xs@exploregroups{\let\@xs@toks0\relax}}

\def\saveexploremode{\let\@xs@saveexploremode\@xs@exploregroups}

\def\restoreexploremode{\let\@xs@exploregroups\@xs@saveexploremode}

% Remplace les #1 premi\`eres occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\@xs@newmacro\StrSubstitute{0}{3}{1}{%
	\def\@xs@reserved@D{#2}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#3}%
	\def\@xs@argument@C{#3}\def\@xs@argument@D{#4}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum#1<\@ne
			\let\@xs@reserved@A\@xs@argument@D
		\else
			\ifnum\decimalpart>#1
				\let\@xs@reserved@A\@xs@argument@C
			\else
				\let\@xs@reserved@A\@xs@argument@D
			\fi
		\fi
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
		\@xs@read@reserved@D
	}%
	\@xs@ifempty{#3}%
		{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#5}%
		}
		{\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#5}%
		}%
}

% Supprime les #1 premi\`eres occurrences de #3 dans #2
\@xs@newmacro\StrDel{0}{2}{1}{\@xs@StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\@xs@exitallgroups{\ifnum\@xs@nestlevel>\z@\endgroup\expandafter\@xs@exitallgroups\fi}

% Compte combien d'unit\'es syntaxiques contient la chaine #1 ?
\@xs@newmacro\StrLen{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\decimalpart\z@
	\let\@xs@nestlevel\z@
	\gdef\groupID{0}%
	\let\@xs@atbegingroup\relax
	\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
	\let\@xs@atnextsyntaxunit\relax
	\@xs@read@reserved@C
	\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n\'ecessaire pour trouver une unit\'e syntaxique derri\`ere
\def\@xs@continuetonext{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel>\z@
			\expandafter\endgroup\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}% on concat\`ene
			\expandafter\expandafter\expandafter\@xs@continuetonext% on recommence
		\fi}
		\relax
}%

\def\@xs@manage@groupID{%
	\begingroup\def\@xs@reserved@A{0}%
	\ifx\@xs@reserved@A\groupID% si on arrive du groupe de niveau 0
		\endgroup
		\xdef\groupID{\number\integerpart}% on met simplement le niveau
	\else
		\endgroup
		\expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\groupID\expandafter\expandafter\expandafter{\expandafter\groupID\expandafter,\number\integerpart}%
	\fi
}

% Cette macro coupe la chaine #1 apr\`es l'unit\'e syntaxique n°#2
\def\StrSplit{%
	\@ifstar
		{\let\@xs@reserved@E\@xs@continuetonext\StrSpl@t}%
		{\let\@xs@reserved@E\relax\StrSpl@t}%
}

\@xs@newmacro\StrSpl@t{}{2}{0}{\@xs@StrSplit@i{#2}{#1}\@xs@StrSplit@ii}

% Cette macro interne coupe la chaine #2 apr\`es l'unit\'e syntaxique n°#1
% Le d\'ebut est assign\'e dans \@xs@reserved@B et la fin dans \@xs@reserved@C
\long\def\@xs@StrSplit@i#1#2{%
	\def\@xs@reserved@D{#1}%
	\def\@xs@reserved@C{#2}%
	\let\@xs@reserved@B\@empty
	\global\let\groupID\@empty
	\ifnum#1>\z@
		\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
			\@xs@read@reserved@C
		}%
		\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
		\def\@xs@atnextsyntaxunit{%
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
			\ifnum\decimalpart=\@xs@reserved@D\relax
				\ifx\@xs@reserved@C\@empty\@xs@reserved@E\fi
				\global\let\@xs@reserved@B\@xs@reserved@B
				\global\let\@xs@reserved@C\@xs@reserved@C
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
}

\def\@xs@StrSplit@ii#1#2{\let#1\@xs@reserved@B\let#2\@xs@reserved@C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\@xs@newmacro*3\StrCut{1}{2}{0}{%
	\@xs@ifempty{#3}%
		{\global\let\groupID\@empty
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		}
		{\ifnum#1<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\@xs@StrCut@ii{#2}{#3}1}
			{\@xs@StrCut@ii{#2}{#3}{#1}}%
		}%
	\@xs@StrCut@iii
}

\long\def\@xs@StrCut@ii#1#2#3{%
	\def\@xs@reserved@D{#1}%
	\let\@xs@reserved@C\@empty
	\def\@xs@reserved@E{#2}%
	\decimalpart\z@\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi
	}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter
	\def
		\expandafter\expandafter\expandafter
	\@xs@reserved@D
		\expandafter\expandafter\expandafter
	{\expandafter\@xs@reserved@C\@xs@argument@A}%
}

\long\def\@xs@StrCut@iii#1#2{\let#1\@xs@reserved@C\let#2\@xs@reserved@E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit\'es syntaxiques aux positions compris !
\@xs@newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\@xs@reserved@E\relax
		\@xs@StrSplit@i{#3}{#1}%
		\edef\@xs@reserved@C{\number\numexpr#2-1}%
		\let\@xs@reserved@E\relax
		\expandafter\expandafter\expandafter\@xs@StrSplit@i\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@B}%
	\expandafter\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
	\global\let\groupID\@empty
}

% supprime #2 unit\'es syntaxiques \`a gauche dans la chaine #1
\@xs@newmacro\StrGobbleLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

% extrait de #1 la chaine \`a gauche de longueur #2
\@xs@newmacro\StrLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% supprime #2 unit\'es syntaxiques \`a droite dans la chaine #1
\@xs@newmacro\StrGobbleRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% renvoie #2 unit\'es syntaxiques \`a la droite de la chaine #1
\@xs@newmacro\StrRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

\@xs@newmacro\StrChar{}{2}{1}{%
	\let\@xs@reserved@B\@empty
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\ifnum#2>\z@
		\def\groupID{0}\let\@xs@nestlevel\z@\integerpart\z@\decimalpart\z@
		\let\@xs@atbegingroup\relax
		\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
		\def\@xs@atnextsyntaxunit{%
			\ifnum\decimalpart=\@xs@reserved@D% la n i\`eme US est atteinte ?
				\global\let\@xs@reserved@B\@xs@reserved@A% on capture l'US en cours qui est celle cherch\'ee
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@B}%
		{\global\let\groupID\@empty}
		\relax
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\@xs@newmacro\StrCount{}{2}{1}{%
	\def\@xs@reserved@D{#1}\def\@xs@reserved@E{#2}\let\@xs@reserved@C\@empty
	\@xs@ifempty{#2}%
		{\@xs@ReturnResult{0}{#3}}
		{\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
			\@xs@read@reserved@D
		}%
		\def\@xs@atoccurfound{\let\@xs@reserved@C\@empty\@xs@read@reserved@D}%
		\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro\StrPosition{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\let\@xs@reserved@E\groupID
	\ifx\@xs@reserved@C\@xs@reserved@D
		\@xs@ReturnResult{0}{#4}%
		\let\@xs@reserved@E\@empty
	\else
		\expandafter\@xs@StrLen\expandafter{\@xs@reserved@C}[\@xs@reserved@C]%
		\expandafter\@xs@ReturnResult\expandafter{\number\numexpr\@xs@reserved@C+1}{#4}%
	\fi
	\global\let\groupID\@xs@reserved@E
}

\def\comparestrict{\let\@xs@comparecoeff\@ne}

\def\comparenormal{\let\@xs@comparecoeff\z@}

\def\savecomparemode{\let\@xs@saved@comparecoeff\@xs@comparecoeff}

\def\restorecomparemode{\let\@xs@comparecoeff\@xs@saved@comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont \'egaux et renvoie la
% position de la premiere unit\'e syntaxiques diff\'erente sinon
\@xs@newmacro*2\StrCompare{}{2}{1}{%
	\def\@xs@reserved@A{#1}%
	\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@B\@xs@reserved@A
		\@xs@ReturnResult{0}{#3}%
	\else
		\def\@xs@next{\@xs@StrCompare@i{#1}{#2}{#3}}%
		\expandafter\@xs@next
	\fi
}

\long\def\@xs@StrCompare@i#1#2#3{%
	\def\@xs@StrCompare@iii##1{%
		\let\@xs@reserved@A\@empty
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@reserved@A{*\@xs@comparecoeff}}%
			{\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
				{\def\@xs@reserved@A{*\@xs@comparecoeff}}
				\relax
			}%
		\def\@xs@next{%
			\expandafter\@xs@ReturnResult\expandafter
			{\number\numexpr##1\@xs@reserved@A\relax}{#3}%
		}%
	}%
	\def\@xs@StrCompare@ii##1{% ##1 est la position
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@B
		\ifx\@xs@reserved@B\@xs@reserved@A
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
				{\@xs@StrCompare@iii{##1}% les 2 unit\'es syntaxiques sont \'egales, on renvoie la position
				}
				{\def\@xs@next{\expandafter\@xs@StrCompare@ii\expandafter{\number\numexpr##1+1}}% les 2 unit\'es syntaxiques sont \'egales et non vides, on recommence
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
				}%
		\else% les 2 unit\'es syntaxiques sont diff\'erentes : on renvoie la position
			\@xs@StrCompare@iii{##1}%
		\fi
		\@xs@next
	}%
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\@xs@StrCompare@ii1%
}

\@xs@newmacro\StrFindGroup{}{2}{1}{%
	\def\@xs@reserved@A{#2}\def\@xs@reserved@B{0}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\def\@xs@next{\@xs@ReturnResult{{#1}}{#3}}%
	\else
		\def\@xs@next{\@xs@StrFindGroup@i{#1}{#2}[#3]}%
	\fi
	\@xs@next
}

\long\def\@xs@StrFindGroup@i#1#2[#3]{%
	\def\@xs@StrFindGroup@ii{%
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@next{\@xs@ReturnResult{}{#3}}% s'il ne reste plus rien, on renvoie vide
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@D
			\ifx\bgroup\@xs@toks% si la 1\`ere unit\'e syntaxique est un groupe explicite
				\advance\decimalpart\@ne% on augmente le compteur
				\ifnum\decimalpart=\@xs@reserved@A% on est au groupe cherch\'e lors de la profondeur courante ?
					\ifx\@empty\@xs@reserved@B% on est \`a la profondeur maximale ?
						\def\@xs@next{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#3}}% on renvoie ce groupe
					\else% sinon
						\expandafter\def\expandafter\@xs@next\expandafter{\expandafter\@xs@StrFindGroup@i\@xs@reserved@D}% on recommence avec ce groupe
						\expandafter\@xs@addtomacro\expandafter\@xs@next\expandafter{\expandafter{\@xs@reserved@B}[#3]}% et les profondeurs de recherche restantes
					\fi
				\else
					\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
					\let\@xs@next\@xs@StrFindGroup@ii
				\fi
			\else
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\let\@xs@next\@xs@StrFindGroup@ii
			\fi
			}%
		\@xs@next
	}%
	\@xs@extractgroupnumber{#2}\@xs@reserved@A\@xs@reserved@B
	\decimalpart\z@
	\ifnum\@xs@reserved@A>\z@\def\@xs@reserved@C{#1}\else\let\@xs@reserved@C\@empty\fi
	\@xs@StrFindGroup@ii
}

\def\@xs@extractgroupnumber#1#2#3{%
	\def\@xs@extractgroupnumber@i##1,##2\@xs@nil{\def#2{##1}\def#3{##2}}%
	\@xs@extractgroupnumber@i#1,\@xs@nil
	\ifx\@empty#3\else\@xs@extractgroupnumber@i#1\@xs@nil\fi
}

\def\expandingroups{\let\@xs@expandingroups\exploregroups}

\def\noexpandingroups{\let\@xs@expandingroups\noexploregroups}

\def\StrExpand{\@testopt{\@xs@StrExpand}{1}}
\long\def\@xs@StrExpand[#1]#2#3{%
	\begingroup
		\@xs@expandingroups
		\ifnum#1>\z@
			\integerpart#1\relax
			\decimalpart\z@
			\gdef\groupID{0}%
			\let\@xs@nestlevel\z@
			\def\@xs@atendofgroup{%
				\expandafter\endgroup
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
				\@xs@read@reserved@C
			}%
			\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
			\def\@xs@atnextsyntaxunit{%
				\expandafter\expandafter\expandafter\@xs@addtomacro
				\expandafter\expandafter\expandafter\@xs@reserved@B
				\expandafter\expandafter\expandafter{\@xs@reserved@A}%
			}%
			\def\@xs@reserved@C{#2}%
			\@xs@StrExpand@i{#1}% Appel de la macro r\'ecursive
		\else
			\def\@xs@reserved@B{#2}%
		\fi
		\global\let\@xs@reserved@B\@xs@reserved@B
	\endgroup
	\let#3\@xs@reserved@B
	\global\let\groupID\@empty
}

\long\def\@xs@StrExpand@i#1{%
	\ifnum#1>\z@
		\let\@xs@reserved@B\@empty
		\@xs@read@reserved@C
		\let\@xs@reserved@C\@xs@reserved@B
		\def\@xs@reserved@A{\expandafter\@xs@StrExpand@i\expandafter{\number\numexpr#1-1}}%
	\else
		\let\@xs@reserved@A\relax
	\fi
	\@xs@reserved@A
}

\def\scancs{\@testopt{\@xs@scancs}{1}}
\long\def\@xs@scancs[#1]#2#3{%
	\@xs@StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

% Restaure le code de @
\catcode`\@=\CurrentAtCatcode\relax

% D\'efinit le d\'elimiteur verb
% d\'efinit les diff\'erents modes et les m\'emorise
\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput
%
% Historique
%------------------------------------------------------------------------------
%% v1.0    4/7/2008 : - Package achev\'e.
%          7/7/2008 : - Package publi\'e sur CTAN.
%------------------------------------------------------------------------------
% v1.1    15/8/2008
%   - Le package ne n\'ecessite plus LaTeX et est d\'esormais utilisable sous
%     Plain eTeX.
%   - Ajout des macros \IfInteger et \IfDecimal.
%     Pour cette derni\`ere, la partie enti\`ere et la partie d\'ecimale sont
%     r\'ecup\'erables dans les compteurs \integerpart et \decimalpart. Ce
%     qu'il reste apr\`es qu'un caract\`ere non attendu soit rencontr\'e est
%     dispo dans \@xs@remainafterdecimal
%   - Correction d'un bug dans \tokenize :
%        suppression de l'expansion avec \normalexpandarg pour \'eviter le bug
%        avec les lettres accentu\'ees dans l'exemple : \tokenize\aa{\'e\`u}
%   - Am\'elioration du code de la plupart des macros.
%   - \'Ecriture d'une routine \@xs@newmacro d\'efinissant les  macros.
%   - Suppression de tous les compteurs grace \`a \numexpr.
%   - Nouvelles fonctionnalit\'es internes dans :
%      \IfSubStr
%        ajout des chaines se trouvant avant et apr\`es l'occurrence test\'ee
%        dans les sc \@xs@behind@IfSubStr et \@xs@before@IfSubStr
%      \StrCount
%        a) ajout de ce qui se trouve apr\`es la derni\`ere occurrence dans la
%           sc \@xs@StrCount@afterlastocccur
%        b) la macro ne d\'epend plus d'aucune autre
%------------------------------------------------------------------------------
% v1.2    23/8/2008
%   - Am\'elioration du code de \StrMid \StrGobbleLeft, \StrLeft,
%     \StrGobbleRight et \StrRight \`a l'aide de la nouvelle macro
%     \@xs@StrSplit@i
%   - Nouveau test \IfStrEq qui compare 2 chaines
%   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
%     contiennent un nombre)
%   - Correction d'un bug dans \@xs@formatnumber. La macro n'envisageait pas le
%     cas o\`u son argument \'etait vide ce qui faiasait planter
%     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
%------------------------------------------------------------------------------
% v1.3    21/9/2008
%  - Am\'elioration du code, mise en place de r\'ecursivit\'es terminales dans
%    toutes les macros r\'ecursives, simplification de \@xs@TestEqual en
%    utilisant \ifx
%  - Nouvelles macros \IfStrEqCase et \IfEqCase
%      Teste si une chaîne est \'egale \`a plusieurs cha\^ines donn\'ee et
%      ex\'ecute un code sp\'ecifique
%  - Cr\'eation de la macro publique \StrSplit
%      Coupe la chaine en 2 \`a une position donn\'ee
%  - Nouvelle macro \StrCompare
%      Compare 2 chaînes et renvoie la position du 1er caract\`ere diff\'erent.
%      Renvoie 0 si elles sont \'egales.
%------------------------------------------------------------------------------
% v1.3a   29/9/2008
%  - Correction d'un bug : \expandafter#1
%    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
%    nombre > 9 !
%  - R\'e \'ecriture de \@xs@returnfirstsyntaxunit et \@gobble qui
%    deviennent purement d\'eveloppables.
%  - R\'e \'ecriture de \StrLen
%  - Nouvelle macro interne \@xs@cutafteroccur
%      Coupe la chaine apr\`es la ni\`eme occurrence d'une sous chaine.
%  - Code am\'elior\'e de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
%    \StrGobbleRight grace \`a \@xs@cutafteroccur
%------------------------------------------------------------------------------
% v1.4   4/11/2008
%  - xstring traite ses arguments par unit\'e syntaxique, et donc toutes les
%    macros internes ont \'et\'e r\'e-\'ecrites \`a cette fin.
%  - Le manuel a \'et\'e r\'e-\'ecrit, rendu plus clair et mieux structur\'e.
%  - Nouvelle fonctionnalit\'e : \expandarg
%      le 1er lex\`eme de chaque argument est 1-d\'evelopp\'e avant que la
%      macro ne soit appel\'ee. Si un argument comporte plus qu'1 lex\`eme,
%      il faut passer par \scancs*[1] pour 1-d\'evelopper toutes les unit\'es
%      syntaxiques.
%  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
%    d\'efaut dans \StrSubstitute et \StrDel
%  - Coh\'erence dans les nom des s\'equences de contr\^oles temporaires qui
%    sont d\'esormais : \@xs@reserved@A \`a \@xs@reserved@E
%------------------------------------------------------------------------------
% v1.4a  12/11/2008
%  - Correction d'un bug dans \@xs@StrSplit dans le cas o\`u l'argument
%     num\'erique est <1 : la 1ere coupure doit être vide et le seconde doit
%     être \'egale \`a l'argument.
%------------------------------------------------------------------------------
% v1.4b  16/11/2008
%  - Correction de 2 bugs dans \@xs@returnfirstsyntaxunit
%------------------------------------------------------------------------------
% v1.5   31/12/2008
%  - Nouvelles fonctionnalit\'es dans la recherche de groupes par un
%    identificateur caract\'erisant leur imbrication. Impl\'ementation de :
%      1) \StrFindGroup
%      2) \groupID
%  - Ajout des nouvelles macros g\'en\'eriques \@xs@read@reserved@C et
%    \@xs@read@reserved@D
%  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
%    que \truc contenait «a{a}».
%  - Correction d'un bug dans \@xs@newmacro : l'argument optionnel \'etait
%    d\'etok\'enis\'e \`a tort dans les macros \'etoil\'ees.
%  - Dans \@xs@newmacro, on doit choisir le num\'ero du dernier argument devant
%    être d\'etok\'enis\'e dans le cas d'une macro \'etoil\'ee (sachant que
%     l'argument optionnel ne l'est jamais)
%------------------------------------------------------------------------------
% v1.5a  09/2/2009
%  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
%    indépendante du mode d'exploration et dispose de ses propres commandes
%    d'exploration : \expandingroups et \noexpandingroups
%  - R\'e-\'ecriture de \scancs, qui devient triviale puisque d\'ependant de
%    \StrExpand. Il n'y a plus de version \'étoil\'ee et d\'esormais, \scancs
%    est sensible au mode d'exploration.
%  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
%  - Correction de bugs : mettre \let\@xs@reserved@E\relax avant d'appeler
%    \@xs@StrSplit@i
%  - Suppression des messages d'erreur, de warning et d'info. xstring devient
%    donc silencieux ;)
%  - Passage de 3 \'a 2 compteurs
%  - Le manuel est d\'esormais plus color\'e, en esp\'erant qu'il sera un peu
%    plus agr\'eable \`a lire !
%------------------------------------------------------------------------------
% v1.5b  13/3/2009
%  - Modification d'un grand nombre de macros de telle sorte que vraiment
%    n'importe quel code peut d\'esormais \^etre plac\'e dans les arguments des
%    macros (comme par exemple des \if, \ifx ou autre, m\^eme sans leur \fi, ce
%    qui n'\'etait pas possible jusqu'alors)
%------------------------------------------------------------------------------
% v1.5c  05/6/2009
%  - Correction d'un bug dans \IfBeginWith : il faut appeler
%    \@xs@returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
%    non pas l'inverse pour que \@xs@toks reflète ce qui se trouve dans #1
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit au cas où #1 commence
%    par un espace : mettre \@xs@toks à 0
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit :
%    \@xs@returnfirstsyntaxunit{{}}\truc
%    faisait que \truc se développait en un espace.
%  - Correction d'un bug dans \@xs@removefirstsyntaxunit où le cas
%    \@xs@removefirstsyntaxunit{ {b}}\truc
%    donnait \truc se développant en «b» au lieu de «{b}».
%------------------------------------------------------------------------------
% v1.5d  28/3/2010
%  - Correction d'un bug dans \IfInteger : \@xs@afterinteger ne donnait pas le
%    bon r\'esultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
%  - \xs@formatnumber ne detokenize plus ses arguments (que m'est-il pass\'e
%    par la t\^ete pour que je code un truc comme ca ?), et donc
%    \@xs@afterinteger et \@xs@afterdecimal ont des tokens ayant le bon
%    catcode
%------------------------------------------------------------------------------
% v1.6  24/10/2012
%  - Correction d'un bug dans \@xs@cutafteroccur au cas o\`u #3<1
%  - \IfDecimal ne \detokenize plus l'argument.
%  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
%    \'etait entre accolades
%  - Nouvelle macro \StrCut
%  - \@xs@cutafteroccur@i ne produit plus d'espace indésirable si #3 était
%    évalué par \numexpr
%------------------------------------------------------------------------------
% v1.7  13/1/2013
%  - Correction d'un manque de rigueur dans les assignations concernant
%    \groupID : elles sont toutes globales d\'esormais
%  - Les macros de xstring sont \long
%------------------------------------------------------------------------------
% v1.7a 28/2/2013
%  - Correction d'un espace parasite dans \@xs@removefirstsyntaxunit
%------------------------------------------------------------------------------
% v1.7b 29/7/2013
%  - La date contenue dans \xstringdate est désormais conforme
%------------------------------------------------------------------------------
% v1.7c 13/10/2013 
%  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
